A Distributed Fair Machine Learning Framework with Private Demographic Data Protection

Fair machine learning has become a significant research topic with broad societal impact. However, most fair learning methods require direct access to personal demographic data, which is increasingly restricted to use for protecting user privacy (e.g. by the EU General Data Protection Regulation). In this paper, we propose a distributed fair learning framework for protecting the privacy of demographic data. We assume this data is privately held by a third party, which can communicate with the data center (responsible for model development) without revealing the demographic information. We propose a principled approach to design fair learning methods under this framework, exemplify four methods and show they consistently outperform their existing counterparts in both fairness and accuracy across three real-world data sets. We theoretically analyze the framework, and prove it can learn models with high fairness or high accuracy, with their trade-offs balanced by a threshold variable.

==> Remove.tex <==


In the sequel, we exemplify how to 
redesign four existing (non-distributed 
non-private) fair learning methods based on 
Algorithm \ref{alg:dfl}. We chose these 
methods because they are fundamental 
and cover different scenarios: 
(i) linear vs non-linear, (ii) 
regression vs classification, 
(iii) predictive learning vs feature learning. 
More sophisticated methods can be redesigned 
in similar ways. For each method, we 
will first revisit its existing design 
and then propose our new design. 

We will write $X$ = $[x_{1}, \ldots, 
x_{n}]^{T}$ as a sample matrix, $Y$ = $[y_{1}, 
\ldots, y_{n}]^{T}$ as the associated label 
vector and $H = [h_{r_{1}}, \ldots, h_{r_{k}}]$ 
as a matrix of returned hypotheses. In addition, 
since $\vec{\alpha} = [\alpha_{1}, \ldots, \alpha_{k}]^{T}$, 
we can write $f = \sum_{t=1}^{k} \alpha_{t} h_{r_{t}} = H \vec{\alpha}$. 

In the following, we propose  four 
distributed fair learning methods and 
contrast them with their existing 
non-distributed counterparts. We 
only label formulas of the proposed methods. 


---- distributed fair ridge regression ----
Calders et al \cite{calders2013controlling} 
developed a fair ridge regression (FRR). 
It minimizes squared loss on training sample, 
while additionally penalizing prediction disparity 
across demographic groups. Let $I_{1}, I_{2}$ be the 
index sets of two demographic groups (e.g. female and male) 
respectively. Their objective function is
\begin{equation*}
J_{FRR}(f) = {\sum}_{i=1}^{n} (f(x_{i}) - y_{i})^{2} 
+ \lambda \cdot \text{MD}(f),     
\end{equation*}
where $\text{MD}(f) = \frac{1}{|I_{1}|} \sum_{i \in I_{1}} 
f(x_{i}) - \frac{1}{|I_{2}|} \sum_{i \in I_{2}} f(x_{i})$ 
is the prediction disparity. 
We see $\min J(f)$ requires simultaneous access 
to $(x,y)$ and $s$; thus this method cannot be directly 
applied in our private learning framework. 

We propose a distributed fair ridge regression 
(DFRR) based on Algorithm \ref{alg:dfl}. 
Our objective function is 
\begin{align}
\begin{split}
 & J_{DFRR}(f) = \sum_{i=1}^{n} (f(x_{i})-y_i)^{2} 
+ \lambda ||f||^{2},\\ 
& \quad\ \ = \sum_{i=1}^{n} \left(
\sum_{t=1}^{k} \alpha_{t} h_{r_{t}}(x_{i}) 
-y_i\right)^{2} 
+ \lambda \left\| \sum_{t=1}^{k} \alpha_{t} 
h_{r_{t}} \right\|^{2}.   
\end{split}
\end{align}
Minimizing the above objective for $\alpha_{t}$'s 
gives 
\begin{equation}
\vec{\alpha} = (H^T X^T X H + \lambda I)^{-1} (H^{T} X^{T} Y).
\end{equation}
The arguments for (2) is simple: 
we first solve for $H \vec{\alpha}$ by standard least 
square method and then for $\vec{\alpha}$. This 
argument will be repeatedly used in the rest  
proposed methods. 
--------------------------------------------------------


---- distributed fair kernel ridge regression ----
Perez-Suay et al\cite{perez2017fair} developed 
a fair kernel ridge regression (FKRR). It minimizes 
squared loss in RKHS while additionally 
penalizing the correlation between prediction and 
demographic feature. Its objective function is 
\begin{equation*}
J_{FKRR}(f) 
= {\sum}_{i=1}^{n} (f(\phi(x_{i})) - y_{i})^{2} 
+ \lambda \Omega(f) + \mu I(f; s),      
\end{equation*}
where $I(f; s) = \sum_{i=1}^{n} 
(\bar{f}(x_{i}) \cdot \bar{s}_{i})$ is 
the correlation between prediction and 
demographic and $\bar{f}$ and $\bar{s}$ 
are centered variables. 
This method also needs 
simultaneous access to $(x,y)$ and $s$. 

We present a distributed fair 
kernel regression (DFKRR) method 
based on Algorithm \ref{alg:dfl}.
Our high-level objective is 
\begin{equation}
J_{DFKRR}(f) 
= \sum_{i=1}^{n} (f(\phi(x_{i}))-y_i)^{2} 
+ \lambda ||f||^{2}.    
\end{equation}
Unlike the standard assumption that $f$ is 
expressed by $\phi(x_{i})$'s, we first assume 
$f$ is expressed by $h_{r_{t}}$'s as in (1) 
and each $h_{r_{t}}$ is linearly 
expressed by $\phi(x_{i})$'s, i.e., 
\begin{equation}
h_{r_{t}} = \sum_{i=1}^{n} c_{ti} \phi(x_{i}),  
\end{equation}
where $c_{ti}$'s are random coefficients 
associated with $h_{r_{t}}$. 
Our assumption is based on an argument that 
if $f$ can be expressed by $\phi(x_{i})$
or $h_{r_{t}}$, then $h_{r_{t}}$ should 
be expressible by $\phi(x_{i})$.\footnote{
A similar assumption is used in \cite{grandvalet2003scaling}
for feature selection in kernel method.} 

Based on (5), we can generate a random hypothesis 
(and its predicted label set) by randomly generating 
a set of associated coefficients. 
Note the coefficients $c_{t_{i}}$'s are known and 
$\alpha_{t}$'s are unknown. Minimizing $J(f)$ gives 
\begin{equation}
\vec{\alpha} = 
 [C^T(K+\lambda I)^{T}(K+\lambda I)C]^{-1}C^{T}(K+\lambda I)^{T}Y.
\end{equation}
where ${K}$ is the Gram matrix and 
$C$ is an $n$-by-$k$ matrix with 
$c_{ti}$ being its element at 
the $i_{th}$ row and $t_{th}$ column. 
---------------------------------------------------------


---- distributed fair logistic regression ----


\hline 

Kamishima et al \cite{kamishima2012fairness} 
developed a fair logistic regression (FGR). 
It maximizes the likelihood of label while 
additionally penalizing mutual information 
between model prediction and demographic 
feature. Its objective function is 
\begin{equation*}
J_{FGR}(f) = - {\sum}_{i=1}^{n} \ln p(y_{i} \mid 
x_{i}, s_{i}, f) + \frac{\lambda}{2} ||f||^{2} + \text{R}(f), 
\end{equation*}
where $\text{R}(f) = \text{E}\, p(f(x),s) \ln 
\frac{p(f(x),s)}{p(f(x)) p(s)}$ measures the 
mutual information and can be estimated from data. 
This method also 
requires simultaneous access to $(x,y)$ and $s$. 

We propose a distributed fair logistic regression 
(DFGR) based on Algorithm \ref{alg:dfl}. 
Our high-level objective function is 
\begin{equation}
\label{eq:dfgr}
J_{DFGR}(f) = - \sum_{i=1}^{n} \ln p(y_{i} 
\mid x_{i}, f) + \lambda ||f||^{2}, 
\end{equation}
where $p(y_{i} | x_{i}, f)$ is constructed 
in the same way as logistic regression, 
with an additional assumption  
$f$ has the form (1). 

Minimizing (\ref{eq:dfgr}) by Newton's method, 
we can update
\begin{equation}
\vec{\alpha} = \vec{\alpha} 
- (J^{''}(f))^{-1} (J^{'}(f)),     
\end{equation}
where
\begin{equation}
J^{'}(f)=H^{T}X^{T}(Y-\vec{p})+2\lambda H^{T}H 
\vec{\alpha},     
\end{equation}
and
\begin{equation}
J^{''}(f)=H^{T}X^{T}MXH+2\lambda H^{T}H,  
\end{equation}
with 
${\vec{p}=[p(f(x_1)=1|x_1;f),
\ldots,p(f(x_n)=1|x_n;f)]^{T}}$ and 
diagonal matrix ${M}$ with 
$M_{ii} = p(f(x_i)=1|x_i;f) 
\cdot p(f(x_i)=0|x_i;f)$ -- both 
are standard quantities in logistic 
regression. 

--------------------------------------------------------

---- fair PCAs ----


\hline 

Samadi et al \cite{samadi2018price} 
developed a fair PCA which minimizes 
reconstruction error while equalizing 
this error across demographic groups. 
Let $X_{1} \in \R^{n_{1} \times p}$ be the 
sample matrix of $n_{1}$ instances in 
one group, $X_{2} \in \R^{n_{2} \times p}$ 
be the sample matrix of $n_{2}$ instances 
in another group, and $V \in \R^{p \times q}$  
be the projection matrix. Their 
objective (to minimize) is 
\begin{equation*}
\max \left\{ \frac{1}{n_{1}} loss(X_{1}, X_{1} V V^{T}), 
\frac{1}{n_{2}} loss(X_{2}, X_{2} V V^{T}) \right\}.  
\end{equation*}
where $loss$ measures reconstruction error. 
Authors show the optimal $V$ gives equal  
reconstruction errors across groups. 

Matt Olfat et al\cite{olfat2018convex} 
proposed another fair PCA method that minimizes 
prediction disparity in the projected space, 
i.e., 
\begin{equation*}
\min_{w, V}\,\sup_t\, | p[w^{T}V^{T}x 
\leq t|s=1]-p[w^{T}V^{T}x \leq t|s=0] |,   
\end{equation*}
where $w$ is the prediction model and $V$ 
is the project matrix. 

Note that both methods need access to $(x,y)$ and $s$. 

We propose a distributed fair PCA (DFPCA) 
method based on Algorithm \ref{alg:dfl}. 
Let $v$ be a projection vector. 
Our optimization probelm is the same as PCA, i.e., 
\begin{equation}
\max_{v} v^T \Sigma_{x} v,  
\quad \text{s.t.} ||v||=1,  
\end{equation} 
where $\Sigma_{x}$ is the covariance matrix. 
Our additional assumption is that $v$ 
is linearly expressed by fair random 
vectors $h_{r_{t}}$, i.e., 
\begin{equation}
v = \alpha_1 h_{r_{1}} + \ldots 
+ \alpha_k h_{r_{k}}  = H \vec{\alpha}. 
\end{equation} 
Solving problem (10) for $\vec{\alpha}$ gives 
\begin{equation} 
H^T \Sigma_{x} H \vec{\alpha} 
= \lambda H^{T} H \vec{\alpha},  
\end{equation}
which implies $\vec{\alpha}$ is the 
leading eigenvector. 

--------------------------------------------------------

--- data set ---


 
The Communities Crime data set contains  
1993 communities, each described by 128 features. 
We selected the fraction of African-American 
residents as the sensitive feature and 
binarized it so that a community is considered 
`minority' if the fraction is above 0.5 and 
`majority' otherwise; the predictive variable 
is the community crime rate that is binarized 
into `high' if rate is above 0.5 and `low' 
otherwise. The COMPAS dataset contains information of 18317 records and 40 features (e.g.Name, race, sex). We filtered 16000 records and 15 numerical features (non-empty). Similar to \cite{chouldechova2017fair}, we select race as the sensitive information and risk of recidivism as the binary prediction variable.

-- experiment observation --

\hline 


Table I shows the classification performance 
of all methods on the Community Crime data set. 


as our empirical studies suggest 
it often leads to efficient accuracy-fairness trade-offs.   

Our first observation is the proposed distributed 
fair learning methods consistently outperform 
their non-distributed counterparts. Take ridge 
regression as an example, DFRR not only achieves 
much lower SP than FRR (0.05 vs 0.31), but 
also simultaneously achieves lower classifier 
error (0.106 vs 0.110) and error parity (0.17 vs 0.23). 
Another example is PCA, where DFPCA achieves 
lower SP than FPCA's (0.03 vs 0.08), lower 
classifier error (0.14 vs 0.15) and lower 
error parity (0.15 vs 0.19). Similar comparisons 
can be observed on most methods across different 
data sets.\footnote{
There are three exceptions: DFGR has higher classifier 
error than FGR on both the Community Crime data set
and the COMPAS data set; DFKRR has slightly 
higher SP than FKRR on the credit data set. However, 
the gaps were mild so we argue our methods are as 
competitive as existing ones.} These observations 
imply that, for fair learning, our proposed $\rho$-fairness 
measure is more efficient than existing ones and our 
proposed learning framework is more effective. 

Our second observation is that the performance gap 
between distributed and non-distributed methods is 
larger for linear models (ridge regression and PCA) 
and sometimes smaller for nonlinear ones 
(e.g. logistic and kernel). 
The former is further backed up by the 
desirable theoretical guarantees we proved for 
linear models. As to why our framework occasionally 
gives less performance improvement on non-linear
base models, we do not have a principled 
hypothesis at the moment. For kernel 
methods, we do make an assumption in 
(5) that a random fair hypothesis can 
be linearly expressed by training instances; 
we suspect this assumption is incorrect 
and needs to be refined. 

Finally, our results suggest fair PCA methods seem less 
effective for classification tasks, as both existing 
methods achieve higher SP and classifier errors 
-- but this is understandable as they are not 
optimized for classification. Again, our proposed 
distributed fair PCA significantly reduces 
SP and classifier error, making itself 
a competitive method for classification tasks  
among other fair classifiers. 

--- figure: sp versus "k" ---

\begin{comment}
\begin{figure}[t!]
\vspace{-10pt}
\centering
  \includegraphics[width=.3\textwidth]{Figures/DFGR.jpg}
  \vspace{-5pt}
  \caption{Classification Performance versus $k$}
  \label{fig:3}
\end{figure}
\end{comment}

--- figure: "k" versus "sigma" ---

\begin{comment}
\begin{figure}[t!]
\vspace{-10pt}
  \centering
  \includegraphics[width=.27\textwidth]{Figures/sigma.jpg}
  \vspace{-5pt}
  \caption{${k}$ versus ${\sigma} $ (fix ${\rho=0.1}$)}
  \label{fig:5}
\end{figure}
\end{comment}


==> Reviewer_Comments.tex <==
\newpage
\section{Comments}

\textbf{Reviewer 1:}

1. Privacy leak is not addressed.
2. Algorithm 1 is not motivated, but it is summarized.
3. What if there are multiple (more than two) parties involved?

\textbf{Reviewer 2:}

1. The proposed framework is not thoroughly described.

2. The relevance in the field of the works used as a comparison in the experiments is not clear.

3. It is not stated if this framework can be applied to other approaches apart from the ones used in the experiments.

*16: Detailed comments for the authors
  In section IV, the authors are supposed to describe their distributed fair learning framework. However, they mainly use this section to describe the redesign of the four non-private fair learning they are using during the evaluation, and barely describing in one paragraph their framework operation. The authors should consider describing their framework more extensively.

Also in section IV, the authors justify the four non-distributed non-private fair learning models chosen for redesign because they are fundamental and cover different scenarios. If they are fundamental works in their respective fields, is there any reason for not introducing them in the state-of-the-art?

In the same vein, it could be relevant knowing which proportion of fair learning models in the literature are suited for your framework redesign. If this proportion is high, it could be an advantage that worth mentioning in the article.

In section VI, the authors present the experiments and their corresponding results. The obtained results are really good as their approach applied to other works shows higher fairness and higher accuracy while providing privacy to sensitive data. Either way, even if the conditions for providing privacy are not met, i.e. data center has all the data, the same process to sensible data can be locally applied; as the resulting learning model seems to have better prediction results. The authors may consider further study of this behavior on further works or on an extension of the article.

It also would be interesting to include some â€œnon-fairâ€ learning models on the experiments. This way the reader will have some reference to determine if the obtained classifier errors are relevant or not. It also could help to evaluate how fairness affects the classifiersâ€™ accuracy.

The article in general is well written, well-structured and easy to follow. It is appreciated the authors wrote it thoroughly. However, there are some typos to correct, these are some of them:
...remove demographic feature from the modelâ€¦
The arguments for (X) is simpleâ€¦
...in algorithm X, and...


==> discussion.tex <==
\section{Discussion}

As future work we identify three important main directions. In the first place we will solve the privacy leakage in the proposed framework, such as, an attacker infers users' sensitive feature by hacking the communication information between the data center and third party. Secondly, we are also interested in redesigning more sophisticated algorithms under our framework rather than the four fair learning methods; For example, redesigning a fair algorithm based on neural network. Finally, we will consider how to extend the proposed framework into multiple parties and generalize the application of this framework. 

==> introduction.tex <==
\section{Introduction}

It is reported that machine learning 
models are giving unfair predictions 
on minority people in consequential 
decision makings. They are biased 
against black defendants in recidivism 
prediction \cite{crime2016bias}, against female 
applicants in job hiring \cite{amazon2018bias} 
and against female employees in facial 
verification \cite{klare2012face}, etc. How to 
learn a fair prediction model 
has become a pressing problem 
in government \cite{prepare2016ai}, 
industry \cite{ms2018biasface,ibm2018biasface} 
and academic \cite{nips2017fair,liu2018delayed, huang2008labeled}. Many fair learning methods are 
developed, from label processing 
\cite{zhang2017anti,luong2011k}  
to feature processing
\cite{feldman2015certifying,zemel2013learning},   
from model regularization 
\cite{dwork2012fairness,zafar2017fairness} 
to model post-processing \cite{hardt2016equality,fish2016confidence} 
-- some have achieved very efficient trade-offs 
between model accuracy and fairness. 

We note that most existing fair learning methods 
require direct access to demographic 
data, e.g., to mitigate racial bias 
a learner needs individual's race information. 
This makes sense, as to measure 
racial bias in prediction, the learner 
needs to first group people based on
race and then compare their predictions. 
However,such demographic data are increasingly 
restricted to use for protecting 
individual privacy. In 2018, Europe launches 
a General Data Protection Regulation 
(GDPR)\footnote{https://eugdpr.org/the-regulation/}. 
It generally prohibits ``processing 
of personal data revealing racial or ethnic original'' and allows users to request 
``erasure of personal data concerning him 
or her'' from the data controller. Besides, 
the privacy research community has a long 
history of hiding sensitive personal data 
from analysis, using techniques such as 
perturbation \cite{agrawal2000privacy,mohammed2011differentially} or encryption \cite{graepel2012ml}. 

We thus see fairness and privacy are running 
in a dilemma in machine learning, i.e., 
most fair learning methods require 
direct access to personal demographic data 
while these data are restricted to use for privacy protection. Debates are arising
\cite{vzliobaite2016using,veale2017fairer}: 
should law permit the use of private demographic 
data for the sake of fair learning? and is it 
technically necessary to have direct access 
to such data? Very few scientific studies 
are done to address these questions. 

In this paper, we propose a distributed fair 
machine learning framework that does not 
require direct access to demographic data. 
Motivated by the ongoing discussions, we 
assume there is a third party that privately 
holds demographic data of the individuals 
being analyzed at data center; to learn 
fair models, the center and party can have
private communications that do not reveal
demographic information. 

We propose a principled way to design fair 
learning methods under the framework. 
Our key insight is as follows: data center 
first constructs a \textit{random but fair
hypothesis space} through private communication 
with the third party; then, it learns an 
accurate hypothesis in this space. 
Our rational is that model fairness is 
ensured as the hypothesis space is fair, 
and model accuracy is promised by random 
projection theory \cite{arriaga2006algorithmic,garg2002generalization}. 
In this paper, we exemplify how to re-design 
four existing fair learning methods: 
fair ridge regression \cite{calders2013controlling}, 
fair kernel regression \cite{perez2017fair}, 
fair logistic regression \cite{kamishima2012fairness} 
and fair PCA \cite{samadi2018price,olfat2018convex}. 
We show the redesigned methods consistently
outperform their counterparts in both 
fairness and accuracy across three 
real-world data sets. 

We also develop a set of theories for the 
proposed distributed and private 
fair learning framework. Under proper 
conditions, we prove the learned model 
is both fair and accurate, and their 
trade-off is indirectly controlled by 
a threshold which used to filter 
hypotheses at the third party. Our 
result also implies one can learn 
a fairer model from a population with 
more balanced demographic distribution. 

The rest of the paper is organized as follows: 
in Section II, we revisit related works; 
in Section III, we introduce notations;  
the proposed framework and exemplified 
methods are presented in Section IV; 
in Section V, we present theoretical results;
experimental results are presented and discussed 
in Section VI, and conclusion is drawn 
in Section VII; In Section VIII, we give out discussion.



==> submission/backup.tex <==




Combine Lemma X and X, we have that 
\begin{equation}
\text{E}[\cov(f(x),s)] \leq 
c_{a} \sigma ||\vec{\cov}(x,s)|| 
\cdot \text{E} (m/k-1)^{-\frac{1}{2}}, 
\end{equation}
which suggests $\rho$-fairness is 
improved at rate $O(\sigma)$. 


% -------  fair kernel method ----------------------
\begin{comment} % 
\begin{equation}
f = \sum_{t=1}^{k} \alpha_{t} 
h_{r_{t}} = \sum_{t=1}^{k} \alpha_{t} 
\sum_{i=1}^{n} c_{ti} \phi(x_{i}) 
= \sum_{i=1}^{n} \tilde{c}_{i} \phi(x_{i}),  
\end{equation}
where $\tilde{c}_{i} 
= \sum_{t=1}^{k} \alpha_{t} c_{ti}$.
Plugging (X) back to (X) gives 
\begin{equation}
J(f) 
= \sum_{i=1}^{n} \left( \sum_{j=1}^{n}
\tilde{c}_{j} k(x_{j},x_{i}) - y_{i} \right)^{2} + \lambda \sum_{i,j=1}^{n} \tilde{c}_{i} 
\tilde{c}_{j} k(x_{i}, x_{j}).
\end{equation}
Solving for $\tilde{c}_{i}$'s and 
then $\alpha_{t}$'s (see Appendix X) gives  
\begin{equation}
(K^{T}K+\lambda K)\tilde{c}=K^{T}Y.
\end{equation}

where $\tilde{c} = C \vec{\alpha}$, then 
\end{comment}
% --------------------------------------------------

% -------  fair logistic regression -----------------
\begin{align}
\begin{split}
J(f) 
& = - \sum_{i=1}^{n} \ln p(y_{i} \mid x_{i}, f) 
+ \lambda ||f||^{2} \\ 
& = \sum_{i=1}^{n} (y_i-1)f(x_i) 
+ \ln[1+\exp(f(x_i))] + \lambda||f||^{2} \\
& = \sum_{i=1}^{n}(y_i-1)\sum_{t=1}^{k}\alpha_{t}h_{r_{t}}(x_i) \\ 
& \quad +\log[1+\exp\sum_{t=1}^{k}\alpha_{t}h_{r_{t}}(x_i)] 
+ \lambda||\sum_{t=1}^{k}\alpha_{t}h_{r_{t}} ||^{2}. 
\end{split}
\end{align}
% --------------------------------------------------


% -------  fair logistic regression -----------------
\subsubsection{Distributed Fair PCA}

We learn a fair projection matrix $V \in \R^{p*k}$ 
which composed by fair vector ${v_i \in R^{p*1}}$. Each ${v_i}$ is linear combination of fair hypotheses  and $\{\alpha_1,\ldots,\alpha_k\}$ are coefficients to be learned. Our objective function is 

\begin{align}
\begin{split}
&\alpha_i= \mathop{\arg\max}_{\alpha_i}(v_i)^T\sum_{cov}v_i \\[.3em]
&\text{s.t.}\  (v_i)^Tv_i=1\\[.3em]
&(v_i)^Tv_j=0 \quad i \neq j
\end{split}
\end{align}

Let fair subspace ${W_{fair} = \{h_{r_1},\ldots,h_{r_k}\}}$, by using the Lagrange multiplier method, we have 

\begin{align}
\begin{split}
(W_{fair})^{T}\sum_{cov}W_{fair}\alpha_i=\lambda_i (W_{fair})^{T}W_{fair}\alpha_i
\end{split}
\end{align}

Let ${P=W_{fair}^T\sum_{cov}W_{fair}}$ and  ${ Q = W_{fair}^TW_{fair}}$, we rewrite formula (21) as

\begin{equation} 
{ P\alpha_i=\lambda_i Q\alpha_i}
\end{equation}

By definition ${\alpha_i}$ is an eigenvector of matrix ${Q^{-1}P}$ and ${\lambda_i}$ is the associated eigenvalue. 
% --------------------------------------------------


% ------ error caused by random projection -----------
\begin{lemma}
Let h be an n-dimensional classifier, $x \in \mathcal{R}^{n}$ a sample point, such that $||h|| 
= ||x|| = 1 $, and $v = h^{T}x.$ Let $R \in \mathcal{R}^{n \times n}$ be a random projection matrix with $h^{'} = Rh, x^{'} = Rx$. Then the probability of misclassifying x, relative to its classification in the original space, due to the random projection, is
\begin{equation}
P[sign(h^{T}x) \neq sign(h^{'T}x^{'})] \le g(\bar{\eta})e^{-\frac{v^{2}k}{8(2+|v|)^{2}}}
\end{equation}

\begin{comment}
where $g(h_{*}) = \frac{4-2c}{4-(2+h_{*})c} 
+ \frac{2+2c}{2+(2+h_{*})c}$.
\end{comment}
\begin{comment}
\begin{equation}
[\big||u^{'}|^{2} - |u^{'}|^{2}\big| \ge c|u|^{2}] 
\le g(h_{*}) e^{-\frac{c^{2}k}{8}}
\end{equation}
\end{comment}
\end{lemma}

\begin{proof}
From Lemma 8, we know that with probability at least $Z(c) = 1 - g(\bar{\eta})e^{-\frac{v^{2}k}{8(2+|v|)^{2}}}$, we have
\begin{equation}
(1-c)||h||^{2} \le ||h^{'}||^{2} \le (1+c)||h||^{2}
\end{equation}
\begin{equation}
(1-c)||x||^{2} \le ||x^{'}||^{2} \le (1+c)||x||^{2}
\end{equation}
\begin{equation}
(1-c)||h-x||^{2} \le ||h^{'}-x^{'}||^{2} \le (1+c)||h-x||^{2}
\end{equation}
Since $||h|| = ||x|| = 1$, and setting $v = h^{T}x, v^{'} = h^{'T}x^{'}$, we have $||h-x|| = ||h||^{2} + ||x||^{2}-2h^{T}x = 2-2v$ and $||h^{'} - x^{'}||^{2} = ||h^{'}||^{2} + ||x^{'}||^{2} - 2v^{'}$. In particular $||h^{'}||^{2} + ||x^{'}||^{2} - 2v^{'} \le (1+c)(2-2v)$ Namely, $v^{'} \ge (||h^{'}||^{2}+||x^{'}||^{2})/2 - (1+c)(1-v) \ge (1-c)-(1+c)(1-c) = c(v-2)+v$. Thus, when $v > 0$ we have $v^{'} > 0$ if $c(v-2)+v \ge 0$. This implies that we need $v/(2-c) > c$. Similarly, $||h^{'}||^{2} + ||x^{'}||^{2} - 2v^{'} \ge (1-c)(2-2v)$. Namely, $v^{'} \le ||h^{'}||^{2} + ||x^{'}||^{2}/2 - (1-c)(1-v) \le 1+c-1+c+v(1-c) = 2c+v(1-c) = c(2-v)+v$. In particular, if $v<0$ then $v^{'}<0$ if $c(2-v)+v \le 0$, which implies $c<-v/(2-v)$.

Then, $c<|v|/(2+|v|)$, we have
\begin{align}
\begin{split}
P[sign(h^{T}x) &\neq sign(h^{'T}x^{'})] \le 1-Z(\frac{|v|}{2+|v|}) \\
&= g(\bar{\eta})e^{-\frac{v^{2}k}{8(2+|v|)^{2}}}    
\end{split}
\end{align}

\end{proof}
% ----------------------------------------------


% ------ generalization error caused by random projection -----------
\begin{lemma}
Regarding to a classifier $h$, a sample $S$, and a random projection matrix $R$, we can define the classification error caused by the projection matrix $R$ as
\begin{equation}
Err_{proj}(h,R,S) = \frac{1}{|S|}\sum_{x\in S}I(sign(h^{T}x \neq sign(h^{'T}x^{'}))
\end{equation}

Let h be an n-dimensional classifier, R a random projection matrix, and a sample of m points

\begin{equation}
S = \{(x_{1}, y_{1}),...,(x_{m},y_{m})|x_{i} \in \mathcal{R}^{n}, y_{i} \in \{0,1\} \}
\end{equation}
Then, with probability $\ge 1-\delta$, the projection error satisfies $Err_{proj}(h,R,S) \le \epsilon_{1}(S,\delta)$, where

\begin{equation}
\epsilon_{1}(S,\delta) = \frac{1}{m}\frac{1}{\delta}\sum_{i=1}^{m}g(\bar{\eta})e^{-\frac{v^{2}k}{8(2+|v|)^{2}}}
\end{equation}
$v_{i} = h^{T}x, for i = 1,...,m.$
\end{lemma}

\begin{proof}
We set Z as the expected projection error of a sample where the expect ion is taken with respect to the choice of the projection matrix. Using Lemma 9, we can get,
\begin{equation}
\begin{split}
Z &= E[Err_{proj}(h,R,S)]  \\
  &= E\bigg[\frac{1}{|S|}\sum_{x\in S}I(sign(h^{T}x) \neq sign(h^{'T}x^{'}))\bigg]  \\
  &= \frac{1}{m}\sum_{x \in S}E\bigg[I(sign(h^{T}x) \neq sign(h^{'T}x^{'}))\bigg]  \\
  &= \frac{1}{m}\sum_{x \in S}Pr \bigg[sign(h^{T}x) \neq sign(h^{'T}x^{'}) \bigg]   \\
  &\le \frac{1}{m} \sum_{x \in S} g(\bar{\eta})e^{-\frac{v^{2}k}{8(2+|v|)^{2}}} = \delta\epsilon_{1}(S,\delta)
\end{split}
\end{equation}
\end{proof}
% ----------------------------------------------


% ------ final error bound ----------
\begin{lemma}
Let S denote a sample of size m from $\mathcal{R}^{n}$. Let h denote the linear classifiers we have. $\bar{E}(h)$ and $\hat{E}(h,s)$ means the expected error and empirical error of a classifier h on the sample set S when the data was sampled according same distribution D.

Assume we observed 2m samples of k dimensional data that can be realized by a k dimensional linear classifier. By using results from \cite{garg2002generalization}, we can conclude with probability not smaller than $1-4\delta$, we have
\begin{equation}
\begin{split}
 \bar{E}(h) &\le \hat{E}(h,s) + 2\epsilon_{1}(S, \delta) \\
 &+ 2\sqrt{\frac{(k+1)ln(2em/(k+1))+ln(1/\delta)}{2m}}  
\end{split}
\end{equation}

From Lemma 10, $\epsilon_{1}(S,\delta) = \frac{1}{m}\frac{1}{\delta}\sum_{i=1}^{m}g(\bar{\eta})e^{-\frac{v^{2}k}{8(2+|v|)^{2}}}$, then we can get
\begin{equation}
\begin{split}
 \bar{E}(h) &\le \hat{E}(h,s) + \frac{2}{m}\frac{1}{\delta}\sum_{i=1}^{2m}g(\bar{\eta})e^{-\frac{v^{2}k}{8(2+|v|)^{2}}} \\
 &+ 2\sqrt{\frac{(k+1)ln(2em/(k+1))+ln(1/\delta)}{2m}}  
\end{split}
\end{equation}
\end{lemma}
% ----------------------------------------------

\begin{equation}
Pr(Y \le (1-c)k) \le \frac{e^{\frac{-\bar{\eta}\lambda}{1+2\lambda}} \cdot e^{\lambda(1-c)k}}{(1+2\lambda)^{k/2}}
\end{equation}
Putting $\lambda = c/2 $ we get $Pr(Y \le (1-c)k) \le e^{\frac{-\bar{\eta} c}{2+2c}-\frac{c^{2}k}{4}}$
We set $P^{'} = Pr(Y \ge (1+c)k)+Pr(Y \le (1-c)k) = Pr(|Y-K| \ge ck) $.
\begin{equation}
\begin{split}
P^{'}  &\le e^{\frac{\bar{\eta} c}{4-2c} - \frac{c^{2}k}{8}} 
+ e^{\frac{-\bar{\eta} c}{2+2c}-\frac{c^{2}k}{4}} \\
&\le  e^{\frac{\bar{\eta} c}{4-2c} - \frac{c^{2}k}{8}} 
+ e^{\frac{-\bar{\eta} c}{2+2c}-\frac{c^{2}k}{8}} \\
&=(e^{\frac{\bar{\bar{\eta}} c}{4-2c}} + e^{\frac{-\bar{\eta} c}{2+2c}})e^{-\frac{c^{2}k}{8}}
\end{split}
\end{equation}

\begin{equation}
P^{'} < g(\bar{\eta})e^{-\frac{c^{2}k}{8}}
\end{equation}
Where $g(\bar{\eta}) = \frac{4-2c}{4-(2+\bar{\eta})c} + \frac{2+2c}{2+(2+\bar{\eta})c}$.Then,

\begin{equation}
Pr[\big||u^{'}|^{2} - |u^{'}|^{2}\big| \ge c|u|^{2}] \le g(\bar{\eta})e^{-\frac{c^{2}k}{8}}
\end{equation}

If $-\frac{2}{c} - 2 < \bar{\eta} 
< \frac{4}{c} - 2$, we have 
\begin{equation}
g(h_{*}) \leq  \frac{4-2c}{4-(2+\bar{\eta})c} + \frac{2+2c}{2+(2+\bar{\eta})c}. 
\end{equation}


% discussion 


\begin{comment}
In compared methods, FGR has best fairness performance on Crime dataset. However,this method is worse than DFGR. FPCA2 presents better fairness and accuracy than FPCA1, as FPCA1 depends on balancing reconstruction loss of subgroups but increasing reconstruction error.The two methods compared with DFPCA, our method has better performance since it maximizes data variance which can maximally preserve the original data structure in the projected space and the dimension reduction is based on numerous fair hypertheses.The statistics of DFRR suggests it has better performance in prediction fairness and accuracy, because this method minimizes prediction error based on numerous fair hypotheses. For non-linear case, it is obvious that kernel method has advantage that prediction error is smaller than linear case,especially when the original dimension of features is high. The statistics of DFKRR shows this method has better fairness and accuracy performance than FKRR when we set the ${\rho=10^{-4}}$.  
\end{comment}


==> submission/removed.tex <==
# Notation Section 

In this paper, we are given a dataset ${X}$ consisting of ${n}$ i.i.d. samples ${\{(S_i,C_i,Y_i)}_{i=1}^n\}$ from a joint distribution ${P}$ with domain ${\mathcal{S
\times C \times Y}}$.Here, ${S \in \mathcal{S}}$ denotes one or more sensitive variables such as gender and race, ${C \in \mathcal{C}}$ denotes other non-sensitive variables used for decision making, and ${Y}$ denotes the true label for a given sample. Each ${x \in X}$ is a vector of length ${D}$ where each component of the vector describes the attributes of the sample. We focus on discrete and finite domains ${\mathcal{S}}$,${\mathcal{C}}$ and ${\mathcal{Y}=\{0,1\}}$ in this paper. There is no restriction on the dimensions of ${S}$ and ${C}$.We use ${\hat{Y}}$ denotes prediction label of a model. The training data and testing data is denoted as ${X_S=[x_S^1,...,x_S^{N_S}] \in R^{D*N_S}}$ and ${X_T=[x_T^1,...,x_T^{N_T}] \in R^{D*N_T}}$,respectively,where${N_S}$ and ${N_T}$ are the number of samples in training set and testing set.
Let ${W \in R^{D*d}}$ represents a basis transformation that would map the training and testing data from the raw space ${R^D}$ to a new space ${R^d}$.The symbol ${(.)^T}$ denotes the transpose operator.The symbol ${||.||_2}$ denotes the ${l_2}$ norm. The notion ${<.,.>}$ to denote the inner product. Throughout this paper,matrix is written in capital letters, and variable is written in lowercase.


# Methodology 

\subsubsection{Fair linear regression}

Supposing data center receives ${m(m>>D)}$ fair feature embedding functions ${\{w_1,w_2,...,w_m\}}$ from third party which ${w_i}$ satisfies ${cov(w_i^Tc,s)\leq \rho}$. Based on the fair base vectors, our goal is to learn a fair linear combination of fair vectors,namely, 
\begin{align}
\begin{split}
W_{fair}=&\beta_{1}w_1 + \beta_{2}w_2+...+\beta_{i}w_i+....+\beta_{m}w_m\\
=& W_{base}*\beta
\end{split} 
\end{align}


Where ${\beta^{T}=[\beta_{1},\beta_{2},...,\beta_{m}]}$ is the cofficient vector and ${W_{base}}$ is composed by fair vectors ${\{w_1,w_2,...,w_m\}}$.

From (1), If $\{w_1,...,w_m\}$ are fair vectors, we can learn a vector ${\beta}$ to obtain  ${W_{fair}}$(Theorem 4.1). Adding the constraint of minimizing prediction error,${W_{fair}}$ will be fair and accurate. Considering the good performance of ridge regression model, we embed fair vectors into this model, then we learn an optimal ${\beta}$ by minimizing the objective function as follows:

\begin{align}
\begin{split}
&\min_{\beta}\sum_{i=1}^{N_S}(x_i^T (W_{base}\beta)-y_i)+\lambda\sum_{k=1}^m\beta_k^2\\[.3em]
&\text{s.t.}\  ||\beta||^{2}_2=1
\end{split} 
\end{align}



In formula (2), the first term is minimizing prediction error, the second term uses L2-regularization, because it helps to reduce model complexity by shrinking regression coefficients.

We apply the Lagrange Multiplier and convert it into an unconstrained optimization problem, then use the critical point method to obtain an optimal solution for optimal ${\beta}$,
\begin{equation} 
 {\beta^{*} = [W_{base}^TX_S^TX_SW_{base}+(\lambda-\gamma) I]^{-1}W_{base}^TX_S^TY}
\end{equation}

Where ${\lambda,\gamma}$ are Lagrange multipliers.

\subsection{Kernel Ridge Regression}





Supposing base vectors $\{\beta_1,...,\beta_m\}$ are fair in kernel space, we can learn a fair linear combination of fair base vectors,namely,
\begin{align}
\begin{split}
\beta = c_1\beta_1+...+c_m\beta_m =\beta^{T}C
\end{split} 
\end{align}

where ${\beta_i}$ is column vector, ${C}$ is coefficient vector. If each ${\beta_i}$ is fair, we can learn a ${C}$ makes ${\beta}$ fair. 

Now, let's discuss the method to obtain fair ${\beta}$.Assuming we have a nonlinear transformation ${\Phi}(x)$ from the original ${D}$ dimensional feature space to an  ${M}$ dimensional
feature space, where ${M>>D}$.The objective function of traditional kernel ridge regression model is:
\begin{align}
\begin{split}
J(\beta) = {\sum}_{i=1}^n(\Phi(x_i)\beta-y_i)^{2}+\lambda \beta^{T}\beta
\end{split} 
\end{align}

By using critical point method, we have 

\begin{align}
\begin{split}
\beta = {\sum}_{i=1}^n-\frac{1}{\lambda}((\Phi(x_i))^{T}\beta-y_i)(\Phi(x_i)={\sum}_{i=1}^n\alpha_i\Phi(x_i)
\end{split} 
\end{align}




Formula (16) suggests the optimal ${\beta}$ is a linear combination of training instances.

We can make prediction on any instance once ${\alpha}$ is obtained,

\begin{align}
\begin{split}
 {\sum}_{i=1}^n\alpha_i\Phi(x_j)^{T}\Phi(x_i)={\sum}_{i=1}^n\alpha_i k(x_j,x_i)
\end{split} 
\end{align}

We let ${\beta_k={\sum}_{i=1}^n \alpha_i^{(k)}\Phi(x_i),k \in [1,m]}$, then we have

\begin{align}
\begin{split}
\Phi(x_j)^{T}\beta =& {\sum}_{k=1}^m c_k{\sum}_{i=1}^n \alpha_i^{(k)}k(x_j,x_i)\\
\end{split} 
\end{align}

Where ${\alpha_i^{(k)}}$ is the ${k}$-th fair vector which returned by third party.

In (19), we learn a vector ${C=\{c_1,...,c_m\}}$ based on numerous fair vectors to make the prediction satisfies ${cov(\Phi(x_j)^{T}\beta,s) \leq \rho}$ (Theorem 4.3). 


\section{Fair Feature Learning}




\subsection{Fair feature learning}
We embedded fair base vectors into traditional PCA to obtain fair feature subspace. First, we give out related theorem and definition:

\begin{definition}
(\textbf{Fair PCA}) Given ${m}$ data points in ${R^{n}}$ with subpopulations $\{S=s\}$ and $\{S=s^{'}\}$, we define fair PCA as finding a fair projection ${h(x) = Wx, W \in R^{d*p}}$ into a ${\rho}$-fair feature subspace ${M}$ to realize ${(\gamma,\epsilon)}$-prediction fairness: ${\gamma = \sup_{h(x)} |\hat{q}_{s\hat{y}M} - \hat{q}_{s^{'}\hat{y}M}| }$ and ${\epsilon = \sup_{h(x)} |1-\frac{\hat{q}_{s^{'}\hat{y}M}}{\hat{q}_{s\hat{y}M}}| }$.
\end{definition}

\begin{theorem}
(\textbf{${\rho}$-fair vector}) If prediction base space ${W_{base}}$ is composed by numerous of fair vector $\{w_i \in R^{D*1}|i \in m\}$, ${m}$ is big enough. We have vector ${\mathcal{V} =W_{base}\beta }$ satisfies ${\rho}$-fair property(proof in Appendix).
\end{theorem}

\begin{definition}
(\textbf{${\rho}$-fair feature subspace}) Let 
${M=(w_1^{*},...,w_k^{*})}$ be composed by ${w_i^{*},i \in [1,k]}$ which is ${\rho}$-fair vector, we say ${M}$ is a ${\rho}$-fair feature subspace,
\begin{align}
\begin{split}
  cov((w_i^{*})^{T}{x},s) \leq \rho \quad for \quad \forall i \in [1,k]
\end{split}
\end{align}
\end{definition}

%------------------updated 05092019-----------
Let ${x_i \in R^D}$ be an instance. ${{W =W_{base}\beta_i}}$ be a ${\rho}$-fair projection vector, ${W_{base} \in R^{D*m}}$ is composed by vector bases in the data center which returned by the third party. We generate a latent feature ${x_i^'}$ by projecting $x_i$ onto ${W}$,

\begin{equation} 
 {x_i^{'} = (W_{base}\beta_i)^Tx_i}
\end{equation}

To learn a ${\beta_i}$ that can maximally preserve the original data structure in the projected space. we maximize data variance.

We let ${W = (W_{base}\beta_i)^T }$, then the data variance in the projected space denoted by:

\begin{align}
\begin{split}
\sum_{x_i^{'}} = E[(x_i^{'}-E[x_i^{'}])^2] 
=\frac{1}{N_S}\sum_{i=1}^{N_S}(W^Tx_i-W^T\mu)(W^Tx_i-W^T\mu)^T
=W^T\sum_{cov} W
\end{split} 
\end{align}

Where ${\sum_{cov}}$ is the covariance matrix and ${\mu}$ is the mean of samples.

We learn ${\beta_1}$ from training data that maximize ${\sum_{x_i^{'}}}$ while restricting ${||W_*^{(1)}||^2 = (W_*^{(1)})^TW_*^{(1)}=1}$ where ${W_*^{(1)} = W_{base}\beta_1}$. Namely,


\begin{align}
\begin{split}
&\beta_1= \mathop{\arg\max}_{\beta_1}(W_*^{(1)})^T\sum_{cov}W_*^{(1)} \\[.3em]
&\text{s.t.}\  (W_*^{(1)})^TW_*^{(1)}=1
\end{split}
\end{align}

By using Lagrange method, we obtain the following formula,

\begin{equation} 
{W_{base}^T\sum_{cov}W_{base}\beta_1=\lambda_1 W_{base}^TW_{base}\beta_1}
\end{equation}

Let ${P=W_{base}^T\sum_{cov}W_{base}}$ and  ${ Q = W_{base}^TW_{base}}$, 
\begin{equation} 
{Q^{-1}P\beta_1=\lambda_1 \beta_1}
\end{equation}

By definition ${\beta_1}$ is an eigenvector of matrix ${Q^{-1}P}$ and ${\lambda_1}$ is the associated eigenvalue. 

After obtaining ${\beta_1}$, the first optimal projection vector is given by using ${W_*^{(1)} = W_{base}\beta_1}$. The later optimal projection vectors are obtained similarly with an additional constraint that the generated features ${W_*^{(i)}x_i}$ and ${W_*^{(j)}x_i}$ are statistical uncorrelated. Thus, we can find ${W_*^{(i)}=W_{base}\beta_i}$ by obtaining ${\beta_i}$ using the following objective function:
\begin{align}
\begin{split}
&\beta_i= \mathop{\arg\max}_{\beta_i}(W_*^{(i)})^T\sum_{cov}W_*^{(i)} \\[.3em]
&\text{s.t.}\  (W_*^{(i)})^TW_*^{(i)}=1\\[.3em]
&  cov(W_*^{(i)}x_i,W_*^{(j)}x_i)=0 \quad i \neq j
\end{split}
\end{align}

After derivation, we can obtain the relation between ${W_*^{(i)}}$ and ${W_*^{(j)}}$,

\begin{equation} 
{cov(W_*^{(i)}x_i,W_*^{(j)}x_i)=0 \quad \longrightarrow \quad (W_*^{(j)})^TW_*^{(i)}=0 }
\end{equation}


Therefore, we rewrite (9) as formula (11):

\begin{align}
\begin{split}
&\beta_i= \mathop{\arg\max}_{\beta_i}(W_*^{(i)})^T\sum_{cov}W_*^{(i)} \\[.3em]
&\text{s.t.}\  (W_*^{(i)})^TW_*^{(i)}=1\\[.3em]
&(W_*^{(j)})^TW_*^{(i)}=0 \quad i \neq j
\end{split}
\end{align}

Applying the Lagrange multiplier method, ${\beta_i}$ can be obtained by using

\begin{equation} 
(W_{base})^T\sum_{cov}W_{base}\beta_i=\lambda_{i}(W_{base})^TW_{base}\beta_i
\end{equation}

At last, we obtain the optimal ${\beta^{*}}$ for fair feature learning:

\begin{equation} 
{\beta^{*} = \{\beta_1,\beta_2,...,\beta_m\}}
\end{equation}

After we obtain the ${\beta = \{\beta_1,...\beta_{m}\}}$, we can obtain ${\rho}$-fair feature subspace ${W_* \in R^{D*m}}$ which composed by ${\{W_*^{(1)},...,W_*^{(m)}\}}$. Based on ${W_*}$, we can make fair prediction by using ridge regression model.

\subsubsection{Fair kernel PCA}

Assuming the projected new features have zero mean,namely, ${{\frac{1}{n}\sum}_{i=1}^{n}\Phi(x_i)=0}$.
The covariance matrix calculated by
\begin{align}
\begin{split}
\sum_{cov}= {\frac{1}{n}\sum}_{i=1}^{n}\Phi(x_i)\Phi(x_i)^{T}
\end{split} 
\end{align}

The ${k}$-th eigenvector of covariance matrix are given by

\begin{align}
\begin{split}
v_k = {\sum}_{i=1}^{n}\alpha_{ki}\Phi(x_i)
\end{split} 
\end{align}

Where ${\alpha_{ki}=\frac{1}{n}\{\frac{1}{\lambda_k}\Phi(x_i)^{T}v_k\}}$ and ${\lambda_k}$ is the ${k}$-th eigenvalue.

In traditional kernel PCA, we obtain ${\alpha_k}$ by using 

\begin{align}
\begin{split}
\frac{1}{n}{\sum}_{i=1}^{n}k(x_l,x_i){\sum}_{j=1}^{n}\alpha_{kj}k(x_i,x_j)=\lambda_k{\sum}_{i=1}^{n}\alpha_{ki}k(x_l,x_i)
\end{split} 
\end{align}

After obtaining ${\alpha_k}$, the resulting kernel principal components can be caculated by
\begin{align}
\begin{split}
y_k(x_j) = \Phi(x_j)^{T}v_k={\sum}_{i=1}^{n}\alpha_{ki}k(x_j,x_i)
\end{split} 
\end{align}

We obtain fair feature space by learning ${\alpha \in R^{n*m}}$ based on numerous fair vectors: Suppose we have fair base space ${W_{base}}$ which is composed by ${m}$ fair vectors, we learn ${\beta}$ by using the same method with linear case, then we obtain fair feature space by using

\begin{align}
\begin{split}
\alpha_k = W_{base}*\beta_k \quad k =1...m
\end{split} 
\end{align}

\begin{definition}
\textbf{(${\rho}$-relevance of variables)}.If the covariance between variables ${X}$ and ${S}$: ${cov(X,S)\leq \rho}$, we say  ${X}$ and ${S}$ is ${\rho}$-relevance. If ${cov(X,S)=0}$,
 we say ${X}$ and ${S}$ are independent.
 
Specifically, in fairness, if${X}$ denotes non-sensitive variable and ${S}$ denotes sensitive variable, we say variable ${X}$ and ${S}$ is ${\rho}$-fair when ${cov(X,S)\leq \rho}$.
\end{definition}


# Theory of Fair Hypothesis Space 


\begin{theorem}
(\textbf{Linear function of ${\rho}$-fair variables}) Assuming ${\{x_1,...,x_m,s\}}$ are ${m+1}$ variables, ${x_i \in \{x_1,...,x_m\}}$ satisfies ${\rho}$-relevance with ${s}$.Let ${\beta^{T}=\{\beta_1,\beta_2,...,\beta_m\}}$ where ${||\beta||^{2}=1}$, we have linear function of ${f(x;\beta)=\beta_1x_1+...+\beta_mx_m}$ satisfies ${\rho}$-fair propertity: ${cov(f(x;\beta),s) \leq \rho}$.
\end{theorem}


\begin{proof}
According to the definition 1, we have ${cov(x_i,s) \leq \rho}$.
\begin{align}
\begin{split}
cov(f(x;\beta),s) =& E[f(x;\beta)\cdot s]-E[f(x;\beta)]E[s]\\
=&E[(\beta_1 x_1+...+\beta_m x_m)\cdot s]-
E[(\beta_1 x_1+...+\beta_m x_m)]E[s]\\
=&E[(\beta_1x_1) \cdot s]+...+E[(\beta_m x_m) \cdot s]-E[s]\{E(\beta_1x_1)+...+E(\beta_m x_m)\}\\
=&\{E[(\beta_1x_1) \cdot s]-E[s]E[(\beta_1x_1] \}+...+\{E[(\beta_m x_m \cdot s]-E[s]E[(\beta_m x_m] \}\\
=&cov(\beta_1 x_1,s)+...+cov(\beta_m x_m,s)
\end{split}
\end{align}
According to the property of covariance: Let $ a_1$, $ a_2$ be scalars, and let $ X$ and $ Y$ be random variables, then ${cov(a_1 X, a_2 Y)=a_1a_2 cov(X,Y)}$. ${\beta_i}$ is a scalar. Hence, we can obtain:

\begin {equation} 
cov(\beta_i x_i,s) = \beta_i cov(x_i,s)
\end {equation}

Based on (36), we rewrite (35) as,
\begin{align}
\begin{split}
cov(f(x;\beta),s)  =& \beta_1 cov(x_1,s)+...+\beta_m cov(x_m,s)
\end{split}
\end{align}
Because ${cov(x_1,s)\leq \rho,...,cov(x_m,s)\leq \rho}$,then 
\begin{align}
\begin{split}
cov(f(x;\beta),s) =& \beta_1 cov(x_1,s)+...+\beta_m cov(x_m,s)\\
\leq & \beta_1 \rho+...+\beta_m \rho\\
\leq & \rho(\beta_1+...+\beta_m)\\
\leq & \rho ||\beta||^{2}\\
\leq & \rho
\end{split}
\end{align}
\end{proof}


# TP notation (seems not so relevant?) 



To ensure prediction fairness and accuracy, we give out theoretical guarantee in this part.




\begin{remark}
We will use notation ${TP_s(\hat{Y})}$ and ${TP_s^{'}(\hat{Y})}$ to refer to the positive rates of ${\hat{Y}}$ on the subpopulations $\{S=s\}$ and $\{S=s^{'}\}$,respectively. ${TP_s(\hat{Y})}$ and ${TP_s^{'}(\hat{Y})}$ are calculated based on the empirical distribution of data.
\end{remark}

\begin{remark}
Let ${\hat{q}_{s\hat{y}} := \hat{P}[\hat{Y}=1|S=s]}$ be the fraction of the data with $\{\hat{Y}=1,S=s\}$, ${\hat{q}_{s^{'}\hat{y}} := \hat{P}[\hat{Y}=1|S=s^{'}]}$ be the fraction of the data with $\{\hat{Y}=1,S=s^{'}\}$. Let ${\hat{q}_s :=\hat{P}[S=s]}$ be the fraction of the data with $\{S=s\}$ and  ${\hat{q}_{s^{'}} :=\hat{P}[S=s^{'}]}$ be the fraction of the data with $\{S=s^{'}\}$.
\end{remark}

\begin{remark}
By using the introduced notation, given a classifier ${\hat{Y}}$
   \begin{equation}
       \hat{q}_{s\hat{y}} = \frac{TP_s(\hat{Y})}{\hat{q}_s} \quad \quad
       \hat{q}_{s^{'}\hat{y}} = \frac{{TP_s^{'}(\hat{Y})}}{\hat{q}_{s^{'}}}
   \end{equation}

\end{remark}

# proof of connection between covariance and DI. SP

\begin{proof}

Let ${X}$ and ${Y}$ are two discrete random variables, we give out the definition of Hoeffding covariance\citep{matula2011generalized}:

\begin{equation}
    Cov_H(X,Y)=\int_{-\infty}^{\infty}\int_{-\infty}^{\infty}H_{X,Y}(x,y)dxdy
\end{equation}
Where ${H_{X,Y}(x,y)=p(X\leq x,Y \leq y)-p(X\leq x)p(Y \leq y)}$. If the usual product moment covariance ${Cov(X,Y)}$ exists,then it is equal to the Hoeffding covariance.

We can obtain the upper bound of ${|H_{X,Y}(x,y)|}$\citep{matula2003some}:

\begin{equation}
    Sup \quad |H_{X,Y}(x,y)| \leq |Cov_H(X,Y)|
\end{equation}

Namely, 
\begin{equation}
    Sup \quad |F_{X,Y}(x,y)-F_X(x)F_Y(y)| \leq |Cov_H(X,Y)|
\end{equation}

Where ${F_{X,Y}(x,y)}$ is the joint distribution function of ${X}$ and ${Y}$. ${F_X(x)}$ and ${F_Y(y)}$ are their marginal distribution functions.

Combing with conditional probability function we can obtain the following inequality formula,

\begin{equation}
    Sup \quad |F_{X,Y}(y|x)-F_Y(y)| \leq |Cov_H(X,Y)|/F_X(x)
\end{equation}

Where ${F_X(x) =\sum_{x_i\leq x}p(x_i),F_Y(y) =\sum_{y_i\leq y}p(y_i)}$ and ${F_{X,Y}(y|x)=p(Y\leq y|X\leq x)}$.

We rewrite (72) as 

\begin{equation}
    Sup \quad |p(Y\leq y|X\leq x)-\sum_{y_i\leq y}p(y_i)| \leq |Cov_H(X,Y)|/\sum_{x_i\leq x}p(x_i)
\end{equation}

Assuming ${Y \in \{0,1\}}$ and ${X \in \{0,1\}}$, let ${y=1}$ and ${x=1}$, according to the (73), we can obtain
\begin{align}
\begin{split}
 Sup \quad |p(Y=1|X=1)+p(Y=1|X=0)-\xi|\leq |Cov_H(X,Y)|
\end{split}
\end{align}
Where ${\xi=1-\sum p(Y=0|X=[0,1])}$

Because ${p(Y=1|X=1) \geq 0}$ and  ${ p(Y=1|X=0) \geq 0}$ then

\begin{align}
\begin{split}
 Sup \quad |p(Y=1|X=1)-p(Y=1|X=0)-\xi| \leq & \\
 Sup \quad |p(Y=1|X=1)+p(Y=1|X=0)-\xi|
 \leq &|Cov_H(X,Y)|
\end{split}
\end{align}

No matter ${\xi}$ is positive or negative number, we can obtain the upper bound of ${|p(Y=1|X=1)-p(Y=1|X=0)|}$:

\begin{align}
\begin{split}
 Sup \quad |p(Y=1|X=1)-p(Y=1|X=0)| \leq &|Cov_H(X,Y)|+|\xi|
\end{split}
\end{align}

When ${Cov_H(X,Y) \leq \rho}$, the left-side of (76) is bounded by ${|\rho|+|\xi|}$.
\begin{align}
\begin{split}
 Sup \quad |1-\frac{p(Y=1|X=0)}{p(Y=1|X=1)}|\leq & 
 Sup \quad |\frac{|Cov_H(X,Y)|+|\xi|}{p(Y=1|X=1)}|\\
 \leq& Sup \quad |\frac{|Cov_H(X,Y)|+|\xi|}{p(Y=1,X=1)}|\\
 \leq & Sup \quad |\frac{|Cov_H(X,Y)|+|\xi|}{p(Y=1)+p(X=1)-1}|
\end{split}
\end{align}
When ${Cov_H(X,Y) \leq \rho}$, the left-side of (77) is bounded by ${|\frac{|\rho|+|\xi|}{p(Y=1)+p(X=1)-1}|}$.
\end{proof}

# repeated theorem on the connection between covaraince and DI

\begin{theorem}
(\textbf{${(\gamma,\epsilon)}$-prediction fairness\quad vs\quad ${\rho}$-fair vector)}. The ${\rho}$-fair vector ${\mathcal{V}}$ guarantees ${(\gamma,\epsilon)}$-prediction fairness with probability at least ${1-\varepsilon}$: Let ${\mathcal{V^{'}}}$ be any ${\rho}$-fair vector and ${\hat{q}_{s\hat{y}}}$, ${\hat{q}_{s^{'}\hat{y}}}$ be the output of classifier ${\hat{Y}}$, we have ${\hat{q}_{s\hat{y}}}$ and ${\hat{q}_{s^{'}\hat{y}}}$ satisfy ${(\gamma,\epsilon)}$-prediction fairness,
\begin{align}
\begin{split}
|\mathcal{V^{'}}(X;\hat{q}_{s\hat{y}})-\mathcal{V^{'}}(X;\hat{q}_{s^{'}\hat{y}})| < \gamma \\
|1-\frac{\mathcal{V^{'}}(X;\hat{q}_{s^{'}\hat{y}})}{\mathcal{V^{'}}(X;\hat{q}_{s\hat{y}})}| < \epsilon
\end{split}
\end{align}
\end{theorem}
\begin{proof}
 
 Supposing we have  ${W_{base}^{'}^{T}=\{w_1^{'},w_2^{'},...,w_m^{'}\}}$ where ${w_i^{'}}$ is basis vector in data center, ${\mathcal{V^{'}}=\beta_1^{'} w_1^{'}+\beta_2^{'} w_2^{'}+...+\beta_m^{'} w_m^{'}=W_{base}^{'}\beta^{'}}$, then 
\begin{align}
\begin{split}
  cov(\hat{y},s) =& cov(\mathcal{V^{'}}^{T}x,s) \\
  =& cov[{(w_1^{'}^{T}\beta_1+w_2^{'}^{T}\beta_2+...+w_m^{'}^{T}\beta_m)x,s}]\\
  =&\beta_1cov((w_1^{'})^{T}x,s)+...+\beta_mcov((w_m^{'})^{T}x,s)\\
  \leq &(\beta_1+\beta_2+...+\beta_m)\rho \\
  \leq &\rho
\end{split}
\end{align}

Because we have proved ${\gamma = \sup |\hat{q}_{s\hat{y}W} - \hat{q}_{s^{'}\hat{y}W}| }$ and ${\epsilon = \sup |1-\frac{\hat{q}_{s^{'}\hat{y}W}}{\hat{q}_{s\hat{y}W}}| }$ based on ${ cov(\hat{y},s) \leq \rho}$. Therefore, 
${|\mathcal{V^{'}}(X;\hat{q}_{s\hat{y}})-\mathcal{V^{'}}(X;\hat{q}_{s^{'}\hat{y}})| < \gamma}$ and ${|1-\frac{\mathcal{V^{'}}(X;\hat{q}_{s^{'}\hat{y}})}{\mathcal{V^{'}}(X;\hat{q}_{s\hat{y}})}| < \epsilon}$ is true.
\end{proof}

# another theory 


\begin{theorem}
(\textbf{${(\gamma,\epsilon)}$-prediction fairness\quad vs\quad ${\rho}$-fair feature subspace)}. The subspace ${M}$ guarantees ${(\gamma,\epsilon)}$-prediction fairness with probability at least ${1-\xi}$(${\xi}$ is very small): Let ${M}$ be any ${\rho}$-fairness feature subspace and ${\hat{q}_{s\hat{y}M}}$, ${\hat{q}_{s^{'}\hat{y}M}}$ be the output of classifier ${\hat{Y}}$, we have ${\hat{q}_{s\hat{y}M}}$ and ${\hat{q}_{s^{'}\hat{y}M}}$ satisfy ${(\gamma,\epsilon)}$-prediction fairness,

\begin{align}
\begin{split}
|\hat{q}_{s\hat{y}M} - \hat{q}_{s^{'}\hat{y}M}|< \gamma \\
|1-\frac{\hat{q}_{s^{'}\hat{y}M}}{\hat{q}_{s\hat{y}M}}| < \epsilon
\end{split}
\end{align}
\end{theorem}

\begin{proof}

Assuming ${x \in R^{p*1}}$,${W \in R^{p*k}}$ and ${\{W^{T}={w_1^{*},...,w_k^{*}}\}}$,${\beta \in R^{k*1}}$, ${\hat{y}}$ is prediction label. The covariance between ${\hat{y}}$ and sensitive feature ${s}$ denoted by $cov(\hat{y},s)$.

\begin{align}
\begin{split}
  cov(\hat{y},s) =& cov((W\beta)^Tx,s) \\
  =& cov[{(w_1^{*}\beta_1+w_2^{*}\beta_2+...+w_k^{*}\beta_k)^{T}x,s}]\\
  =&\beta_1cov((w_1^{*})^{T}x,s)+\beta_2cov((w_2^{*})^{T}x,s)+...+\beta_kcov((w_k^{*})^{T}x,s)\\
  \leq &(\beta_1+\beta_2+...+\beta_k)\rho 
\end{split}
\end{align}

Because ${||\beta||_2^{2}=1}$,${\beta_1^{2}+...+\beta_k^{2}=1}$, ${(\beta_1+\beta_2+...+\beta_k)< 1}$, then
${cov(\hat{y},s) \leq \rho}$. Based on theorem 4.4, we have ${|\hat{q}_{s\hat{y}M} - \hat{q}_{s^{'}\hat{y}M}|< \gamma}$ and ${|1-\frac{\hat{q}_{s^{'}\hat{y}M}}{\hat{q}_{s\hat{y}M}}| < \epsilon}$.
\end{proof}



# proof of returned fair embedding functions. 

\begin{proof}

 By using Gaussian tail inequality, we have
 
\begin{align}
\begin{split}
p(X > \mu+\rho) \leq \exp^{\frac{-\rho^2}{2\sigma^2}} \quad for \quad \rho \geq 0
\end{split} 
\end{align}

Then, we have 
\begin{align}
\begin{split}
p(X \leq \mu+\rho) \geq 1-\exp^{\frac{-\rho^2}{2\sigma^2}} \quad for \quad \rho \geq 0
\end{split} 
\end{align}

for 
\begin{align}
\begin{split}
p(\rho \leq X \leq \rho+\mu) =& \int_\rho^{\rho+\mu} \frac{1}{\sqrt{2\pi\sigma^2}}\exp^{-\frac{(x-\mu)^2}{2\sigma^2}}dx\\
\leq& \int_\rho^{\rho+\mu} \frac{1}{\sqrt{2\pi\sigma^2}}\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}dx\\
=&\frac{\mu}{\sqrt{2\pi\sigma^2}}\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}
\end{split} 
\end{align}

\begin{align}
\begin{split}
p(X < \rho) =& p(X \leq \mu+\rho)-p(\rho \leq X \leq \rho+\mu)\\
\geq & 1-\exp^{\frac{-\rho^2}{2\sigma^2}}-\frac{\mu}{\sqrt{2\pi\sigma^2}}\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}\\
\geq & 1-\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}-\frac{\mu}{\sqrt{2\pi\sigma^2}}\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}\\
=&1-(1+\frac{\mu}{\sqrt{2\pi\sigma^2}})\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}
\end{split} 
\end{align}

Let ${\frac{M}{N}=p(X <\rho)}$, then we prove theorem 4.9.

\end{proof}



# proof of fair PCA 

\begin{proof}

If ${h^{'}(x) = W^*x}$ be a solution to the fair PCA problem, according to the definition of fair PCA, ${W^*} \subseteq M $. Because ${M}$ is a ${\rho}$-fair feature subspace, ${W^*}$ is also a ${\rho}$-fair feature subspace,i.e.,

\begin{align}
\begin{split}
  cov((w_j^{*})^{T}{x},s) \leq \rho \quad for \quad \forall j \in [1,d]
\end{split}
\end{align}

If ${W^*}$ is a ${\rho}$-fair feature subspace, according to theorem 4.6, we have ${\gamma = \sup_{h^{'}(x)} |\hat{q}_{s\hat{y}W^*} - \hat{q}_{s^{'}\hat{y}W^*}| }$ and ${\epsilon = \sup_{h^{'}(x)} |1-\frac{\hat{q}_{s^{'}\hat{y}W^*}}{\hat{q}_{s\hat{y}W^*}}| }$.
\end{proof}



# fair learner design strategy 

{\color{red} 

I suggest using an Algorithm Enviroment to describe 
the framework here. 
}

1. Data center randomly generates $m$ hypotheses 
$h_{1}, \ldots, h_{m}$ and applies each to separately 
label the training set. For $h_{k}$, we have a 
predicted label set 
$\hat{Y}_{k} = \{ h_{k}(x_{1}), \ldots, h_{k}(x_{n}) \}$.

2. Data center sends $\hat{Y}_{1}, \ldots, \hat{Y}_{m}$ 
to the third party. 

3. Third party evaluates the covariance between 
each $\hat{Y}_{k}$ and the demographic set $S = 
\{ s_{1}, \ldots, s_{n} \}$ and returns index 
$k$ if $cov[\hat{Y}_{k}, S]$ is small (e.g. 
smaller than a threshold $\rho)$. 

4. Data center receives a set of returned 
indices $r_{1}, \ldots, r_{k}$. 

5. Data center learns an accurate model $f$ 
assuming it has the form  
$f = \alpha_{1} h_{r_{1}} + \ldots 
+ \alpha_{r_{k}} h_{r_{k}}$, where 
$\alpha_{r_{1}}, \ldots, \alpha_{r_{k}} \in \R$ 
are unknown coefficients to be learned. 



# insight summary 

We have two major insights that guarantee the success 
of the proposed design strategy: (1) any hypothesis 
spanned by a set of fair hypotheses remains fair;   
(2) with high probability, one can find an accurate
hypothesis in a randomly projected space (based 
on the random projection theory). 
In section \ref{sec:theory}, we will use these 
insights to derive upper bounds on the fairness 
and accuracy of a hypothesis learned under the 
DFL framework. 


# fair kernel regression 

Let $\phi(x)$ be the image of instance 
$x$ through a feature mapping function 
$\phi$. Kernel ridge regression finds 
an $f$ that minimizes 
\begin{equation}
J(f) = \sum_{i} [f(\phi(x_{i}) - y_{i}]^{2} 
+ \lambda ||f||^{2}. 
\end{equation}
By the Representer theorem, the optimal 
$f$ is $f = \sum_{i} c_{i} \phi(x_{i})$ 
for some coefficients $c_{i}$'s (to be 
learned). Plugging this back to $J(f)$ 
gives the dual form 
\begin{equation}
J(c) = \sum_{i} [ \sum_{j} c_{j} k(x_{j},x_{i}) 
- y_{i}]^{2} + \lambda \sum_{i,j} c_{i} c_{j} 
k(x_{i}, x_{j}).  
\end{equation}
One can solve $\min_{c} J(c)$ for $c_{i}$'s. 

To implement a fair kernel ridge regression 
under the DFL framework, we assume the optimal 
$f$ has the form 
$f =\sum_{t=1}^{k} \alpha_{t} h_{r_{t}}$.
Based on [X], we further assume each base 
vector $h_{r_{t}}$ has the form 
\begin{equation}
h_{r_{t}} = \sum_{i=1}^{n} c_{ti} \phi(x_{i}). 
\end{equation}
Now we can generate a random 
$h_{r_{t}}$ by generating 
a set of random coefficients 
$\{\tau_{ci}\}_{i=1,\ldots,n}$. 
The optimal $f$ is 
\begin{equation}
f = \sum_{t=1}^{k} \alpha_{t} 
h_{r_{t}} = \sum_{t=1}^{k} \alpha_{t} 
\sum_{i=1}^{n} c_{ti} \phi(x_{i}) 
= \sum_{i} \tilde{c}_{i} \phi(x_{i}),  
\end{equation}
where 
\begin{equation}
\tilde{c}_{i} = \sum_{t} 
\alpha_{t} c_{ti}.     
\end{equation}
Plugging this back to $J(f)$ gives 
the dual form 

When making prediction on any instance, we have 
\begin{equation}
f(\phi(z)) 
= \sum_{i} \tilde{c}_{i} \phi(x_{i}) \phi(z) 
= \sum_{i} \tilde{c}_{i} k(x_{i}, z).  
\end{equation}

# 

\begin{theorem}
Assuming variable ${X :=cov(w_i^Tc,s)}$ and ${X}$ is distributed with mean ${\mu}$ and variance ${\sigma^{2}}$, ${X \sim N(\mu,\sigma^2)}$. If data center produce ${N}$ functions randomly, then the third party receive ${M}$ fair vectors at least which satisfy ${cov(w_i^Tc,s) < \rho}$. The quantitative relation between ${M}$ and ${N}$ satisfies: ${M > \lfloor N*(1-\frac{\mu+\sqrt{2\pi}\sigma}{\sqrt{2\pi}\sigma}\exp^{{-\frac{(\rho-\mu)^{2}}{2\sigma^{2}}}})\rfloor}$.
\end{theorem}

# theorem 

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}  
\renewcommand{\algorithmicensure}{\textbf{Output:}} 
\newcommand{\theHalgorithm}{\arabic{algorithm}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\newenvironment{proof}[1][Proof]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{definition}[1][Definition]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}


# fair PCA

\subsection{Fair Feature Learning}

\textcolor{red}{describe fair PCA.}

\begin{definition}
(\textbf{Fair PCA}) Given ${m}$ data points in ${R^{n}}$ with subpopulations $\{S=s\}$ and $\{S=s^{'}\}$, we define fair PCA as finding a fair projection ${h(x) = Wx, W \in R^{d*p}}$ into a ${\rho}$-fair feature subspace ${M}$ to realize ${(\gamma,\epsilon)}$-prediction fairness: ${\gamma = \sup_{h(x)} |\hat{q}_{s\hat{y}M} - \hat{q}_{s^{'}\hat{y}M}| }$ and ${\epsilon = \sup_{h(x)} |1-\frac{\hat{q}_{s^{'}\hat{y}M}}{\hat{q}_{s\hat{y}M}}| }$.
\end{definition}

\begin{theorem}
Let ${h^{'}(x) = W^*x}$ be a solution to the fair PCA problem, then we have:

(1) ${W^*=[w_1^*,w_2^*,...,w_d^*](d<p)}$ is a ${\rho}$-fair feature subspace.

(2) ${\gamma = \sup_{h^{'}(x)} |\hat{q}_{s\hat{y}W^*} - \hat{q}_{s^{'}\hat{y}W^*}| }$ and ${\epsilon = \sup_{h^{'}(x)} |1-\frac{\hat{q}_{s^{'}\hat{y}W^*}}{\hat{q}_{s\hat{y}W^*}}| }$.
\end{theorem}


# proof of bounds of K

Assuming variable ${X :=cov(f(x),s)}$ and ${X}$ is distributed with mean ${\mu}$ and variance ${\sigma^{2}}$, ${X \sim N(\mu,\sigma^2)}$. Data center produce ${N}$ hypotheses randomly.

By using Gaussian tail inequality, we have

\textcolor{red}{I'm not completely 
following the proof, e.g., the second 
line of (24) and Let's discuss it today.}
 
\begin{align}
\begin{split}
p(X \leq \mu+\rho) \geq 1-\exp^{\frac{-\rho^2}{2\sigma^2}} \quad for \quad \rho \geq 0
\end{split} 
\end{align}

for 
\begin{align}
\begin{split}
p(\rho \leq X \leq \rho+\mu) =& \int_\rho^{\rho+\mu} \frac{1}{\sqrt{2\pi\sigma^2}}\exp^{-\frac{(x-\mu)^2}{2\sigma^2}}dx\\
\leq& \int_\rho^{\rho+\mu} \frac{1}{\sqrt{2\pi\sigma^2}}\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}dx\\
=&\frac{\mu}{\sqrt{2\pi\sigma^2}}\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}
\end{split} 
\end{align}

\begin{align}
\begin{split}
p(X < \rho) =& p(X \leq \mu+\rho)-p(\rho \leq X \leq \rho+\mu)\\
\geq & 1-\exp^{\frac{-\rho^2}{2\sigma^2}}-\frac{\mu}{\sqrt{2\pi\sigma^2}}\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}\\
\geq & 1-\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}-\frac{\mu}{\sqrt{2\pi\sigma^2}}\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}\\
=&1-(1+\frac{\mu}{\sqrt{2\pi\sigma^2}})\exp^{-\frac{(\rho-\mu)^2}{2\sigma^2}}
\end{split} 
\end{align}
Let ${\frac{k}{N}=p(X <\rho)}$, then we prove theorem 2.




# theory 


Note that $|u^{'}|^{2} = \sum_{i}^{k}(\mathcal{R}_{t}^{T}u)^{2}$. If each entry of $\mathcal{R}$ is chosen from $N(\bar{\eta}_{i},1)$, then the random variables $\mathcal{R}_{t}^{T}u$ are also normally distributed (and identical), and their sum is a random variable which has the Chi-squared distribution with k degrees of freedom. For simplicity, let $Y = \frac{k}{|u|^{2}}|u^{'}|^{2}$. Then $Y$ can be seen as the sum of squares of $k$ random variables each of which is distributed according to $N(\bar{\eta}_{i},1)$. As such it has the moment generating function


\begin{equation}
f(\lambda) = \mathbf{E}(e^{\lambda Y}) = \frac{e^{\frac{\bar{\eta} \lambda}{1-2\lambda}}}{(1-2\lambda)^{k/2}}   \ \  \lambda < 1/2
\end{equation}


\begin{theorem}
The statistical parity [X] of $f$ is 
\begin{equation}
SP(f \mid s) = |p(f(x) = 1|s=1)-p(f(x)=1|s=0)|.  
\end{equation}
and 
\begin{equation}
DI(f \mid s) = 
\left|1-\frac{p(f(x)=1|s=1)}{p(f(x)=1|s=0)} \right|. 
\end{equation}
If $f$ is $\rho$-fair with respect to $s$, 
we have 
\begin{equation}
SP(f \mid s) \leq  \min \{1,\frac{|\rho|}{p_0p_1}\}  
\end{equation}
and 
\begin{equation}
DI(f \mid s) \leq \min \{1, \frac{|\rho|}{p_0p_1\cdot(p(Y=1)-p_1)}  \}
\end{equation}
Where ${p_0=p(s=0),p_1=p(s=1)}$.

Note: the upper bounds depend on ${\rho}$.
\end{theorem}


==> submission/table_results_temp.tex <==
\begin{table}[htbp]
\caption{Group fairness and accuracy comparison on Crime dataset}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Method} & \textbf{\textit{SP(Crime)}}& \textbf{\textit{DI(Crime)}}& \textbf{\textit{APE(Crime)}} \\
\hline
 PCA   & 0.4409 & 0.6536&0.1455  \\ \hline
 FPCA1 & 0.0859 & 0.3546&0.1747\\ \hline
 FPCA2  & 0.0608 & 0.3319 &0.1602\\ \hline
 LFR  \\ \hline
 RLR  &0.0898 & 0.1154 &0.1166 \\ \hline
 RFC  & 0.0372  & 0.1314 &0.1541\\ \hline
 \textbf{FRR}  & 0.0253 &  0.0667&0.1165\\ \hline
 \textbf{DFFL(FPCA)}  & 0.0289 &  0.0757&0.1170\\ \hline
 \textbf{FLR}   \\ 
\hline
\end{tabular}
\label{tab1}
\end{center}
\end{table}


\begin{table}[htbp]
\caption{Group fairness and accuracy comparison on Credit dataset}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Method} & \textbf{\textit{SP( Credit)}}& \textbf{\textit{DI( Credit)}}& \textbf{\textit{APE(Credit)}} \\
\hline
 PCA   &0.0630 &0.1526&0.3969  \\ \hline
 FPCA1 &0.1833 &0.1458&0.5009\\ \hline
 FPCA2  & 0.0981 &0.1027&0.3000\\ \hline
 LFR  &0.1534 &0.2011&0.4772\\ \hline
 RLR  &0.0779 &0.1283&0.2412 \\ \hline
 RFC  &0.1024 &0.1205&0.3403\\ \hline
 \textbf{FRR}  & 0.0316&0.0754&0.2208\\ \hline
 \textbf{DFFL(FPCA)}  & 0.0167&0.1048&0.2264\\ \hline
 \textbf{FLR}  &0.0118  &0.0913 &0.2244 \\ 
\hline
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{table}[htbp]
\caption{Error gap on Crime dataset}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Method} & \textbf{\textit{Minority}}& \textbf{\textit{Majority}}& \textbf{\textit{Gap}} \\
\hline
 PCA & 0.3436 &  0.1176  &0.2260  \\ \hline
 FPCA1 & 0.3200 &   0.1356  &0.1844\\ \hline
 FPCA2  &0.3119  & 0.1268  &0.1851\\ \hline
 LFR  &0.2351 &  0.1083 &0.1268\\ \hline
 RLR  & 0.2488  & 0.1064  &0.1424 \\ \hline
 RFC  &  0.3071 &  0.1224 &0.1847\\ \hline
 \textbf{FRR}  &0.2284  & 0.1159 &0.1125\\ \hline
 \textbf{DFFL(FPCA)}  &0.2191 &0.1119  &0.1072\\ \hline
 \textbf{FLR}  &0.2335 &0.1123 & 0.1212 \\ 
\hline
\end{tabular}
\label{tab1}
\end{center}
\end{table} 
 
\begin{table}[htbp]
\caption{Error gap on Credit dataset}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Method} & \textbf{\textit{Minority}}& \textbf{\textit{Majority}}& \textbf{\textit{Gap}} \\
\hline
 PCA &0.4534 &0.3852&0.0682 \\ \hline
 FPCA1 & 0.5109 &0.4737& 0.0372\\ \hline
 FPCA2  & 0.3565 &0.2902& 0.0663\\ \hline
 LFR  &0.4831 &0.4360&0.0471 \\ \hline
 RLR   &0.2658 &0.2405 &0.0253 \\ \hline
 RFC  &0.3747 &0.3321&0.0426 \\ \hline
 \textbf{FRR}  & 0.2288 &0.2135&0.0153 \\ \hline
 \textbf{DFFL(FPCA)}  & 0.2484 &0.2221& 0.0263\\ \hline
 \textbf{FLR}  &0.2372&0.2267 &0.0105 \\
\hline
\end{tabular}
\label{tab1}
\end{center}
\end{table} 

\begin{table}[htbp]
\caption{FKRR and FKPCA vs. Standard kernel methods on Crime dataset}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Method} & \textbf{\textit{SP(Crime)}}& \textbf{\textit{DI(Crime)}}& \textbf{\textit{APE(Crime)}} \\
\hline
  KPCA &0.0152 &0.1994 &0.0620\\ \hline
 FKPCA &0.0138 &0.1360 &0.0480\\
\hline
\end{tabular}
\label{tab1}
\end{center}
\end{table} 

\begin{table}[htbp]
\caption{FKRR and FKPCA vs. Standard kernel methods on Credit dataset}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Method} & \textbf{\textit{SP(Crime)}}& \textbf{\textit{DI(Crime)}}& \textbf{\textit{APE(Crime)}} \\
\hline
 KRR   &0.0182 & 0.1619&0.2150\\ \hline
 FKRR & 0.0085& 0.0957&0.1823\\ \hline
 KPCA &0.0217 & 0.0947&0.2478\\ \hline
 FKPCA &0.0209&0.0724 &0.2095\\
\hline
\end{tabular}
\label{tab1}
\end{center}
\end{table} 


In table 1, we show the results of SP,DI and APE for all models. The value of ${\rho=0.01 }$ for Crime dataset and ${\rho=0.25}$ for Credit dataset.We record the average value of 50 epoches for our model. We abbreviate fair ridge regression and fair logistic regression model as FRR and FLR,respectively.



   From table 1 and table 2, we see FRR and DFFL(FPCA) models have better performance in fairness and accuracy than other compared methods when we set the value of ${\rho}$ is 0.01 and 0.25,respectively,especially in improving fairness. On crime dataset, the fairness values of RFC method are 0.0372 and 0.1314, which is best compared with other four methods, but FRR can improves fairness to 0.0253 and 0.0667;FPCA2 presents good performance in fairness(0.0608 and 0.0981), it also worse than our method.FPCA1 has good fair results but its accuracy is worse than traditional PCA, because this method balance reconstruction loss of subgroups but increase reconstruction error.The statistics of FRR suggests it has the best performance in prediction fairness and accuracy,
   because this model minimize prediction error based on numerous fair vectors.Even through the performance of DFFL(FPCA) is a little higher than FRR, but the improvement of fairness and accuracy is obvious than other six methods.By comparing with RLR and FLR, we observed fairness of FLR is more superior and just sacrifice little accuracy.
   
   Next, we show the mis-prediction error rate gap between two subgroups(Crime dataset(Majority vs. minority);Credit dataset(low education vs. high education)) in table 3 and 4.
  
  
 
 
From table 3 and 4, we observed there is huge gap between the PCA's mis-prediction rate for Minority and for Majority on Crime dataset (or for the high educated and for the low educated on Credit dataset);this should not be too surprising because PCA method only making dimensionality reduction by maximizing variance or minimizing reconstruction error without fairness consideration. The other five methods (FPCA1,FPCA2,LFR,RFC,RLR) reduces the gap slightly, and we believe this is because fairness mechanism works. Comparatively,the FRR and DFFL(FPCA) methods manage to reduce the gap effctively, DFFL(FPCA) decreases the gap of 0.2260 to 0.1072 on Crime dataset and FRR also decreases the gap of 0.0682 to 0.0153 on Credit dataset.The root reason is the two methods make prediction based on fair vectors, if the covariance between non-sensitive features and sensitive features is small enough, the prediction will virtually fair.

In order to deal with non-linear case, we extend our linear models to non-linear setting. Table 5 and 6 show the results of FKRR and FKPCA models (for 50 epoches),compared with standard kernel methods. We abbreviate Kernel ridge regression and Kernel PCA as KRR and KPCA respectively in table 5 and 6.



   Compared with table 1 and table 2, it is obvious that kernel method has advantage that prediction error is smaller than linear case. This is because data becomes more separable in higher dimension space. According to the data in table 3, we observed FKRR and FKPCA have slight improvement in fairness and accuracy. There are two reasons: First, the accuracy in kernel space is high so that it won't do too much work even we increase the number of base vectors; Secondly, the prediction in kernel space is based on Gram matrix rather than the original features of data, so the fair vector has smaller effect than linear case.

==> theory.tex <==

\section{Theoretical Analysis}
\label{sec:theory}

In this section, we show 
theoretical results for Algorithm \ref{alg:dfl}.
In addition to the general setting, 
several results are developed for 
linear models and thus applicable on 
DFRR and DFPCA. All results are presented 
in the context of Algorithm \ref{alg:dfl}; 
all proofs are presented in the Appendix. 

\subsection{Preliminaries}

Let $(x,s)$ be a random instance. 
We say $f$ is \textit{$\rho$-fair} with 
respect to $s$ if 
\begin{equation}
|\cov[f(x), s]| \leq \rho.     
\end{equation}
We see the returned hypotheses 
$h_{r_{1}}, \ldots, h_{r_{k}}$ are 
all $\rho$-fair. 

We will show a connection between $\rho$-fairness 
and \textit{statistical parity} (SP) \cite{mcnamara2017provably}, a popular 
fairness measure defined as
\begin{equation}
\SP (f) = |p(f(x)=1|s=1)-p(f(x)=1|s=0)|.  
\end{equation}

To establish the connection, we will use 
a generalized covariance inequality 
\cite[Theorem 2]{matula2003some} 
and its adopted quadrant dependence assumption.
Two random variables $X$ and $Y$ are said to be 
\textit{positively quadrant dependent (PQD)} 
 if, for all $x, y$, there is 
 $\Pr (X \leq x, Y \leq y) \geq \Pr(X \leq x) 
\Pr(Y \leq y)$; they are said to be 
\textit{negatively quadrant dependent (NQD)} 
if the inequality is reversed. The 
inequality is stated as follows. 

\begin{lemma}[Matula'03, Thm2] 
Let $X, Y$ be two PQD or NQD random integers.  
Let $F_{X,Y}(x,y)$ be their joint CDF 
and $F_{X}(x)$, $F_{Y}(y)$ be their 
marginal CDF respectively. 
Let 
\begin{equation}
\cov_H(X,Y) = \int_{-\infty}^{\infty}
\int_{-\infty}^{\infty} \Delta F_{X,Y}(x,y) dxdy,   
\end{equation}
be their Hoeffding covariance\footnote{Hoeffding
covariance, whenever exists, equals the standard
covariance.}, where 
\begin{equation}
\Delta F_{X,Y}(x,y) = F_{X,Y}(x,y) - F_{X}(x) F_{Y}(y).     
\end{equation}
If $\cov_H(X,Y)$ is bounded, then 
\begin{equation}
\sup_{x,y} |\Delta F_{X,Y}(x,y)| 
\leq |\cov_H(X,Y)|.
\end{equation}
\end{lemma}


\vspace{5pt} 

We will develop a generalization error 
bound for Algorithm \ref{alg:dfl} 
based on random 
projection theories. To that end, we 
define a \textit{soft threshold policy} 
for the third party, as an alternate 
to the current policy that returns 
$t$ if $|\cov(h(x_{t}),s)| \leq \rho$.  
Let $h_{*}$ be an ideal hypothesis 
with $\cov(h_{*}(x),s) = 0$. 
A {soft threshold policy} 
returns $t$ of $h_{t}$ with probability 
\begin{equation}
\mathcal{N}(\vec{h}_{*}(x), 
\sigma^{2}_{2} I),     
\end{equation}
where $\vec{h}_{*}(x)$=$[h_{*}(x_{1}), 
\ldots, h_{*}(x_{n})]^{T}$ and 
$\sigma_{2}$ is any constant. 

\subsection{Results on $\rho$-fairness}

In this section, we present theoretical 
results on $\rho$-fairness. 

Our first result shows a hypothesis 
spanned by fair hypotheses remain fair 
-- this is the insight that 
motivates the study. 
\begin{lemma}
\label{lemma_fairF}
If $||\vec{\alpha}|| \leq c_{a}$, 
then $f$ is $(\sqrt{k}\, c_{a} 
\rho)$-fair w.r.t. $s$. 
\end{lemma}

The lemma suggests $\rho$-fairness 
can be improved by choosing a smaller 
$\rho$ in Algorithm 1, and the 
improvement is at rate $O(\rho)$; 
another way is to regularize  
$||\vec{\alpha}||$ --  
in our proposed methods, this is 
done indirectly via regularizing 
$||f||$.\footnote{In experiments, 
we observe indirect regularization 
is better than direct one. }

The lemma also suggests smaller 
$k$ leads to fairer model. 
In Algorithm \ref{alg:dfl}, we only 
control $\rho$ but not $k$. Our 
second result quantifies their relation 
and shows $k$ shall not be too small. 

\begin{lemma}
\label{lemma_k}
Let $(x,s)$ be a random instance 
and $h$ be a random hypothesis. 
The number of returned hypotheses 
$k$ satisfies 
\begin{equation}
\text{E}\, [k] \geq m \cdot 
(1 - \text{E}\, [\cov(h(x),s)]\, / \rho^{2}),   
\end{equation}
where the expectations are taken over 
the randomness of $h$, and the covariance 
is defined over the randomness of $(x,s)$. 
Further, if $h$ is linear and generated 
from $\mathcal{N}(0, \sigma^{2} I)$, then 
\begin{equation}
\text{E}\, [k] \geq m 
\cdot ( 1 - \sigma^2 
||\vec{\cov}(x,s)||^2 / \rho^2),
\end{equation}
where $\vec{\cov}(x,s)$=$\sum_{j=1}^{p} 
\cov(x_{j},s)$ and $x_{j}$ is 
$j_{th}$ entry of $x$.
\end{lemma}

Lemma 3 has two results: one for general 
models and the other for linear models. 
The first result shows bigger $k$ 
(more returned hypotheses) is implied by 
smaller $\text{E} [\cov(h(x),s)]$ 
or bigger $\rho$. The former makes sense, 
since larger expected covariance implies more 
hypotheses are fair and thus should be returned. 
However, this insight is not very actionable 
as long as $h$ is random. The latter suggests 
that hypotheses are removed at rate $O(1/\rho^{2})$, 
and one can collect more hypotheses by 
increasing $\rho$. 
The second result shows bigger $k$ 
is implied by smaller $\sigma^{2}$. 
We have not yet found a good explanation 
for this dependence, but we also observe 
it in experiments. 

Our last result for $\rho$-fairness 
is its connection to statistical parity. 
It is developed based on Lemma 1 
and we will assume $f(x)$ and $s$ are 
PQD or PND. This dependence assumption 
has been widely used in research,  
e.g., \cite{denuit2004nonparametric, dhaene2014multivariate,racine2015mixed}.  
Although we cannot prove its validity, 
we will show empirical evidence that 
$\cov(f(x),s)$ $\geq$ $0$ (which implies 
PQD/PND) in most cases and thus the assumption
is reasonable. 
Our result is as follows. 

\begin{theorem}
\label{thm_sp}
Suppose $f(x)$ and $s$ are PQD or NQD random 
variables with bounded covariance. 
If $f$ is $\rho$-fair w.r.t. $s$, then 
\begin{equation}
\SP(f) \leq  \rho / s_{0} s_{1},    
\end{equation} 
where $s_{0} = p(s=0)$ and $s_{1} = p(s=1)$.
\end{theorem}

Theorem 4 suggests that $\rho$-fairness implies 
statistical parity under mild conditions, 
and one can improve $\SP (f)$ at a rate 
of $O(\rho)$ -- same as the rate of improving 
$\rho$-fairness. 

An interesting insight is that the upper 
bound of $\SP$ achieves it minimum value 
$\rho / s_{0} s_{1}$ $\geq$ $4\rho$ 
at $s_{0}$ = $s_{1}$ = $0.5$. 
This suggests if the population has 
a balanced demographic distribution, 
we can expect to learn a fair model 
with small $\SP(f)$. 

\subsection{Results on Generalization Error}

In this section, we present theoretical 
results on the error. 

Our backbone technique is a random projection 
theory \cite{garg2002generalization} 
which states that data distance 
is likely to be preserved in a randomly projected 
space and thus a model's generalization error 
(based on data distance) is also likely to be preserved. 

To apply the theory, we will assume $f$ is linear 
and thus the returned hypotheses $h_{r}$'s are linear. 
We will interpret $h_{r}$'s as basis of a random space, 
where $h_{r_{k}}(x)$ is $k_{th}$ feature of $x$.\\  
The challenge is that most studies assume 
$h_{r}$'s are drawn from zero-mean normal 
distributions, whereas in Algorithm 1 they 
are not -- they are first drawn from 
zero-mean Gaussian but then selected  
at the third party. 

To bridge the gap, we will use the 
alternate soft threshold policy in (18). 
It is easy to verify that $h_{r_{t}}$ 
is now generated from a Gaussian centered 
at $\vec{h}_{*}$, since it is first drawn 
from a Gaussian and then selected by 
another Gaussian. 
Similar to most studies, we assume 
w.l.o.g. that $h_{r}$ has unit variance  

Our first result extends a data distortion 
bound in \cite{arriaga2006algorithmic} 
from zero-mean distribution to non-zero 
mean distribution.  

\begin{lemma}
\label{lemma_distortion}
Let $x$ be any point and $H = [h_{r1}, \ldots, 
h_{r_{k}}]$ be a projection matrix with each 
projection vector $h_{r_{t}}$ taken
from a normal distribution 
$\mathcal{N}(h_{*}, I)$. 
Let $\tilde{x} = \frac{1}{\sqrt{k}}(H^{T} x)$ 
be the projection of $x$ by $H$. 
We have for $0 \leq c < 1$, 
\begin{equation}
\Pr\{ |\,||\tilde{x}||^{2} - ||x||^{2}\,|
\geq c ||x||^{2}\} \leq g(x) \cdot e^{- 
\frac{c^{2} k }{8}},   
\end{equation}
where $g(x) = 
e^{\frac{ ck \langle h_{*}, x\rangle^{2}}{4 
- 2c}} + e^{\frac{- c k \langle h_{*},
x\rangle^{2}}{2 + 2c}}$. 
\end{lemma}

Compared to the original bound, ours  
has an additional $g(x)$ introduced by 
the non-zero mean $h_{*}$. One can 
further bound $g(x)$ for any $x$. 
We keep it as a function of 
$x$ for later use. 
Nevertheless, it shall not be hard to see 
$g(x)$ is small when $||h_{*}||$ is small. 
In particular, if $h_{*} = 0$, then $g(x) = 2$ 
and we recover the original bound. 

Applying Lemma 5 to re-develop the 
generalization error bound in random 
space \cite{garg2002generalization}, 
we obtain the following result. 

\begin{theorem}
\label{thm_error}
Suppose Algorithm 1 adopts 
the soft threshold policy. 
Let $er(f)$, $\hat{er}(f)$ 
be the expected and empirical 
error of $f$ respectively. 
If $f$ is linear and 
$||f|| = ||x|| = 1$, then 
with probability at least $1-4\delta$, 
\begin{equation}
er(h) \leq \hat{er}(h) + 
 T + \frac{4}{n\delta} 
\sum_{i=1}^{n} g(x_{i}) e^{\frac{- k \langle 
f, x_{i} \rangle^{2}}{8(2+||\langle f, x_{i} 
\rangle||)^{2}}}, 
\end{equation}
where  $T = 2\sqrt{
 \frac{ (k+1) \log (en/(k+1)) 
 + \log 1/\delta}{n} }$ and 
\begin{equation}
g(x_{i}) = e^{\frac{ c_{i} k \langle h_{*}, 
x_{i} \rangle^{2}}{4 - 2c_{i}}} 
+ e^{-  \frac{c_{i} k \langle h_{*}, 
x_{i} \rangle^{2}}{2 + 2c_{i}}}     
\end{equation} 
with $c_{i} = |\langle f, x_{i} \rangle| 
/ (2 + |\langle f, x_{i} \rangle|)$.
\end{theorem}

In the theorem, a critical component 
is $k$. We will interpret its impact 
by refining the bound. 
Define  
\begin{equation}
G_{i}(k) = g(x_{i}) \cdot e^{\frac{- k \langle 
f, x_{i} \rangle^{2}}{8(2+||\langle 
f, x_{i} \rangle||)^{2}}}.     
\end{equation}

Note if $h_{*}$=$0$, then $g(x_{i})$ 
= $0$ and $G_{i}(k)$ = $2 e^{\frac{- 
k \langle 
f, x_{i} \rangle^{2}}{8(2+||\langle 
f, x_{i} \rangle||)^{2}}}$. We see 
$G_{i}(k)$ decreases exponentially 
as $k$ increases. This implies 
that collecting more returned 
hypotheses is an efficient way 
to reduce generalization error. 
We can implement this by choosing 
a bigger $\rho$, based on Lemma 3.
However, Lemma 2 suggests this 
will weaken the $\rho$-fairness 
guarantee.  
Therefore, we see Algorithm 1 
establishes a trade-off between 
accuracy and fairness through 
the choice of $\rho$. 

The case of $h_{*}$ $\neq$ $0$ is  
complicated. We focus on identifying 
conditions that can recover the same 
impact as in the first case. 
Merging the two terms in $G(x_{i})$, 
we have 
\begin{equation}
G_{i}(k) = e^{k L_{1}} + e^{- k L_{2}}, 
\end{equation}
$L_{1}$=$\frac{ c_{i} \langle h_{*}, 
x_{i} \rangle^{2}}{4 - 2c_{i}}$-$\frac{ \langle 
f, x_{i} \rangle^{2}}{8(2+||\langle 
f, x_{i} \rangle||)^{2}}$,\, $L_{2}$=$\frac{c_{i} 
\langle h_{*}, x_{i} \rangle^{2}}{2 + 2c_{i}}$+$\frac{\langle 
f, x_{i} \rangle^{2}}{8(2+||\langle 
f, x_{i} \rangle||)^{2}}$.

Clearly $L_{2} \geq 0$. So the impact of $k$ 
on $e^{- k L_{2}}$ is the same as the case 
of $h_{*}=0$. 
For $L_{1}$, after long (and tedious) elementary 
arguments, we manage to identify a condition that 
$L_{1} \leq 0$ if 
\begin{equation}
\left(\langle h_{*}, x_{i} \rangle^{2} 
- 1/4 \right)  
(||\langle f, x_{i} \rangle|| - 2 )^{2} + 1 \leq 0. 
\end{equation}
Thus if $||\langle h_{*}, x_{i} \rangle|| \leq 1/2$ 
or $||h_{*}|| \leq 1/2$, we have 
$L_{1} < 0$ and overall $G_{i}(k)$ 
decreases exponentially as $k$ increases. 

When condition (27) is not satisfied, however, 
we can easily get an upper bound of $G_{i}(k)$ 
that suggests the opposite, i.e., $G_{i}(k)$ decreases 
exponentially as $k$ decreases. 

The conflicting observations seem to suggest that 
there is an optimal $k$ in between for minimizing 
the generalization error. Due to the time and space 
limits, we leave it as a future study on how to 
identify the optimal $k$ for distributed fair learning. 

